Newborn Be star systems observed shortly after mass transfer

Many classical Be stars acquire their very rapid rotation by mass and angular-momentum transfer in massive binaries. Short-lived intermediate-phase objects have only been discovered recently. Data archives and the literature have been searched for additional candidates exhibiting this patterns. Thirteen candidates were identified at various confidence levels. Adding to the two known systems identified as classical Be star+pre-subdwarf binaries (LB-1 and HR6819), two more (V742Cas, HD44637) could be confirmed with interferometry, with V742Cas setting a new record for the smallest visually observed angular semi-major axis, at a=0.663mas. Two further ones (V447Sct, V1362Cyg) are not resolved interferometrically, but other evidence puts them at the same confidence level as LB-1. V2174Cyg is a candidate with very high confidence, but was not observed interferometrically. The remaining ones are either candidates with varying levels of confidence. Of a mostly magnitude complete sample of 328 Be stars, 0.5-1% are found to have recently completed the mass overflow that led to their formation. Another 5% are systems with compact subdwarf companions, i.e., further evolved after a previous overflow, and possibly two more percent harbor white dwarfs. All these systems are of early B-subtypes, however, and if the original sample is restricted to early subtypes (136 objects), these percentages increase by a factor of about 2.5, while dropping to zero for the mid and late subtypes (together 204 objects). This strongly suggests that early- vs. mid- and late-type Be stars have differently weighted channels to acquire their rapid rotation, namely binary interaction vs. evolutionary spin-up.

==> macros_tri.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       Own macros
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%       Astronomical Variables and Observables 
%
%\newcommand{\mstar}{\mbox{$M_{\star}$}\xspace}
%\newcommand{\rstar}{\mbox{$R_{\star}$}\xspace}
%\newcommand{\req}{\mbox{$R_{\rm eq}$}\xspace}
%\newcommand{\rpole}{\mbox{$R_{\rm pole}$}\xspace}
%\newcommand{\lstar}{\mbox{$L_{\star}$}\xspace}
%
%\newcommand{\teff}{\mbox{$T_{\mathrm{eff}}$}\xspace}
%\newcommand{\logg}{\mbox{$\log g $}\xspace}
%\newcommand{\logeps}{\mbox{$\log\varepsilon$}\xspace} 
%\newcommand{\mdot}{\mbox{$\dot{M}$}\xspace}
%\newcommand{\vsys}{\mbox{$v_{\mathrm{sys}}$}\xspace}
%\newcommand{\vrad}{\mbox{$v_{\mathrm{rad}}$}\xspace}
%\newcommand{\vpuls}{\mbox{$v_{\mathrm{puls}}$}\xspace}
%\newcommand{\vred}{\mbox{$v_{\mathrm{red}}$}\xspace}
%\newcommand{\vviolet}{\mbox{$v_{\mathrm{violet}}$}\xspace}
%\newcommand{\vinf}{\mbox{$v_\infty$}\xspace}
%\newcommand{\vesc}{\mbox{$v_{\mathrm{esc}}$}\xspace}
%\newcommand{\vsini}{\mbox{$v\sin i$}\xspace}
%\newcommand{\vrot}{\mbox{$v_{\mathrm{rot}}$}\xspace}
%\newcommand{\vcrit}{\mbox{$v_{\mathrm{crit}}$}\xspace}
%\newcommand{\vkep}{\mbox{$v_{\mathrm{orb}}$}\xspace}

%\newcommand{\omeang}{\mbox{$\omega$}\xspace}
%\newcommand{\omelin}{\mbox{$\Upsilon$}\xspace} % as in Cranmer, 2006
%\newcommand{\omeorb}{\mbox{$W$}\xspace}

%\newcommand{\wlam}{\mbox{$W_{\lambda}$}\xspace}
%\newcommand{\wlam}{\mbox{$\mathit{EW}$}\xspace}
%\newcommand{\la}{\mbox{$\lambda$}\xspace}
%\newcommand{\bz}{\mbox{$\langle{B_z}\rangle$}\xspace}

%\newcommand{\vr}{\mbox{$V\!/R$}\xspace}
%\newcommand{\bminv}{\mbox{$B\!-\!V$}\xspace}
%\newcommand{\uminb}{\mbox{$U\!-\!B$}\xspace}
%\newcommand{\vminr}{\mbox{$V\!-\!R$}\xspace}
%
%        Astronomical units
%
%\newcommand{\Mstar}{\mstar}   % Not a unit, but a normalization quantity
%\newcommand{\Rstar}{\rstar}   % Not a unit, but a normalization quantity
% Let's do as if the following were SI units  (i.e. in roman):
%\newcommand{\Msun}{\mbox{${\mathrm M}_{\odot}$}\xspace}
%\newcommand{\Rsun}{\mbox{${\mathrm R}_{\odot}$}\xspace}
%\newcommand{\Lsun}{\mbox{${\mathrm L}_{\odot}$}\xspace}
%\newcommand{\Myr}{\mbox{${\mathrm M}_{\odot}{\mathrm{yr}}^{-1}$}\xspace}
% SI units:
%\newcommand{\micron}{\mbox{$\mu\rm m$}\xspace}
%\newcommand{\gcm}{\mbox{$\rm g\,cm^{-3}$}\xspace}
%\newcommand{\kms}{\mbox{${\mathrm{km\,s}}^{-1}$}\xspace}
%
%\renewcommand{\deg}{\degree\xspace}
%
%       Spectral lines, ions and spectral types
%
%\newcommand{\LyB}{\mbox{{{Ly}}$\mathrm{\beta}$}\xspace}
%\newcommand{\HA}{\mbox{{H}$\mathrm{\alpha}$}\xspace}
%\newcommand{\HB}{\mbox{{H}$\mathrm{\beta}$}\xspace}
%\newcommand{\HG}{\mbox{{H}$\mathrm{\gamma}$}\xspace}
%\newcommand{\HD}{\mbox{{H}$\mathrm{\delta}$}\xspace}
%\newcommand{\HE}{\mbox{{H}$\mathrm{\epsilon}$}\xspace}
%\newcommand{\BrG}{\mbox{{Br}$\mathrm{\gamma}$}\xspace}
%\newcommand{\Pa}[1]{\mbox{{Pa}$_{#1}$}\xspace}
%
\newcommand{\spec}[3]{\mbox{#1\,{\sc #2}\,$\lambda$#3}\xspace}
%\newcommand{\specs}[3]{\mbox{#1\,{\sc #2}\,$\lambda\lambda$#3}\xspace}
%\newcommand{\ion}[2]{\mbox{#1\,{\sc #2}}\xspace}
%
%\newcommand{\spt}[2]{\mbox{#1\,#2}\xspace}
%
%       Objects
%
%\newcommand{\alpara}{\mbox{$\mathrm{\alpha}$}~Ara\xspace}
%\newcommand{\alperi}{\mbox{$\mathrm{\alpha}$}~Eri\xspace}
%\newcommand{\betcep}{\mbox{$\mathrm{\beta}$}~Cep\xspace}
%\newcommand{\betlyr}{\mbox{$\mathrm{\beta}$}~Lyr\xspace}
%\newcommand{\gamcas}{\mbox{$\mathrm{\gamma}$}~Cas\xspace}
%\newcommand{\delsco}{\mbox{$\mathrm{\delta}$}~Sco\xspace}
%\newcommand{\omeori}{\mbox{$\mathrm{\omega}$}~Ori\xspace}
%\newcommand{\mucen}{\mbox{$\mathrm{\mu}$}~Cen\xspace}
%\newcommand{\etacen}{\mbox{$\mathrm{\eta}$}~Cen\xspace}
%\newcommand{\lameri}{\mbox{$\mathrm{\lambda}$}~Eri\xspace}
%\newcommand{\omecma}{\mbox{$\mathrm{\omega}$}~CMa\xspace}
%\newcommand{\kapcma}{\mbox{$\mathrm{\kappa}$}~CMa\xspace}
%\newcommand{\epscap}{\mbox{$\mathrm{\epsilon}$}~Cap\xspace}
%\newcommand{\zettau}{\mbox{$\mathrm{\zeta}$}~Tau\xspace}
%\newcommand{\phiper}{\mbox{$\mathrm{\varphi}$}~Per\xspace}
%\newcommand{\piaqr}{\mbox{$\mathrm{\pi}$}~Aqr\xspace}
%\newcommand{\psiper}{\mbox{$\mathrm{\psi}$}~Per\xspace}
%\newcommand{\feper}{\mbox{$48$}~Per\xspace}
%\newcommand{\felib}{\mbox{$48$}~Lib\xspace}
%\newcommand{\betcmi}{\mbox{$\mathrm{\beta}$}~CMi\xspace}
%\newcommand{\delcen}{\mbox{$\mathrm{\delta}$}~Cen\xspace}
%\newcommand{\etatau}{\mbox{$\mathrm{\eta}$}~Tau\xspace}
%\newcommand{\kapdra}{\mbox{$\mathrm{\kappa}$}~Dra\xspace}
%\newcommand{\pcar}{\mbox{$\mathrm{p}$}~Car\xspace}
%\newcommand{\alpcol}{\mbox{$\mathrm{\alpha}$}~Col\xspace}
%\newcommand{\xioph}{\mbox{$\mathrm{\chi}$}~Oph\xspace}
%\newcommand{\upscyg}{\mbox{$\mathrm{\upsilon}$}~Cyg\xspace}
%\newcommand{\betpsc}{\mbox{$\mathrm{\beta}$}~Psc\xspace}
%\newcommand{\omicas}{\mbox{$\mathrm{\omicron}$}~Cas\xspace}
%\newcommand{\sixcep}{\mbox{$\mathrm{6}$}~Cep\xspace}
%\newcommand{\omiaqr}{\mbox{$\mathrm{\omicron}$}~Aqr\xspace}
%\newcommand{\thecrb}{\mbox{$\mathrm{\vartheta}$}~CrB\xspace}
%\newcommand{\onedel}{\mbox{$1$}~Del\xspace}
%\newcommand{\betmon}{\mbox{$\beta^1$}~Mon\xspace}
%\newcommand{\omecar}{\mbox{$\omega$}~Car\xspace}
%
% Codes, Models, Instruments
%
%\newcommand{\bruce}{{\sc bruce/kylie}\xspace}
%\newcommand{\hdust}{{\sc hdust}\xspace}
%\newcommand{\fastrot}{{\sc fas\-trot}\xspace}
%\newcommand{\charron}{{\sc charron}\xspace}
%\newcommand{\bedisk}{{\sc bedisk}\xspace}
%\newcommand{\simeca}{{\sc simeca}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%   Fancy stuff 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\lgrey{\color{black!30!white}}
%\def\grey{\color{black!60!white}}
%\def\green{\color{green}}
%\def\textgreen{\color{ForestGreen}}
%\def\black{\color{black}}
%\def\red{\color{red}}
%\def\blue{\color{blue}}
%\def\yellow{\color{yellow}}
%\def\white{\color{white}}
%\def\magenta{\color{magenta}}
%\definecolor{beige}{HTML}{FFDF8C}
%\def\beige{\color{beige}}
%\def\gold{\color{Olive}}
%
%\newcommand{\draft}[1]{{{\bf\sf\red Draft:}\grey\sf\ #1}\xspace}
%\newcommand{\TRi}[1]{{{\bf\sf\red Rivi:}\grey\sf\ #1}\xspace}
%\newcommand{\TRi}[1]{{{}}}


